Microwave Spectro-Polarimetry of Matter and Radiation across Space and Time

This paper discusses the science case for a sensitive spectro-polarimetric survey of the microwave sky. Such a survey would provide a tomographic and dynamic census of the three-dimensional distribution of hot gas, velocity flows, early metals, dust, and mass distribution in the entire Hubble volume, exploit CMB temperature and polarisation anisotropies down to fundamental limits, and track energy injection and absorption into the radiation background across cosmic times by measuring spectral distortions of the CMB blackbody emission. In addition to its exceptional capability for cosmology and fundamental physics, such a survey would provide an unprecedented view of microwave emissions at sub-arcminute to few-arcminute angular resolution in hundreds of frequency channels, a data set that would be of immense legacy value for many branches of astrophysics. We propose that this survey be carried-out with a large space mission featuring a broad-band polarised imager and a moderate resolution spectro-imager at the focus of a 3.5m aperture telescope actively cooled to about 8K, complemented with absolutely-calibrated Fourier Transform Spectrometer modules observing at degree-scale angular resolution in the 10-2000 GHz frequency range. We propose two observing modes: a survey mode to map the entire sky as well as a few selected wide fields, and an observatory mode for deeper observations of regions of specific interest.

==> fts.tex <==
%----------------------------------------------------------------------
%
% Sub-section for absolute spectrophotometry
% Al Kogut/GSFC
%
%----------------------------------------------------------------------

Order-of-magnitude improvements to current upper limits 
for CMB spectral distortions
require continuous spectra
at modest spectral resolution,
covering 6 or more octaves in frequency
with part-per-million channel-to-channel calibration stability.
Fourier transform spectroscopy is ideally suited 
to this task.
%An optical phase delay between
%one beam directed to the sky
%and a second beam terminated by a blackbody calibrator
%generates an interference fringe pattern
%which may be sampled as a function of phase delay.
%The Fourier transform of the resulting interferogram
%yields the difference spectrum between the sky and the %calibrator.
The FTS measures the difference spectrum between the sky and a blackbody calibrator.
Unlike an imager,
whose frequency channels are set by bandpass filters,
the central frequency,
channel bandwidth,
and channel-to-channel covariance
of an FTS's synthesized frequency channels
depend only on the sampling (apodization)
of the interferograms 
and can be determined {\it a priori}.
The photon noise to first order
is the same for all channels;
it depends on the integrated optical load over the total passband
and scales linearly with the synthesized channel width.

A broad-band Fourier transform spectrometer (FTS)
based on the \PIXIE design\cite{Kogut2011PIXIE}
would achieve the science goals
outlined above.
\PIXIE uses a single FTS with 15 GHz channels
extending from 15 GHz to 6 THz.
If foregrounds were negligible,
\PIXIE could detect the $\mu$-distortion
from Silk damping of primordial density perturbations
at 2--3 standard deviations
and detect recombination lines at comparable levels.
Astrophysical foregrounds degrade the ideal performance
and require additional sensitivity 
at both low and high frequencies \citep{abitbol_pixie}.

Additional sensitivity may be obtained
using several nearly-identical FTS modules,
each with a different optical passband
and different synthesized frequency channels,
optimized for either the CMB distortion signals
or the measuring the competing foreground emission.
Table~\ref{tab:fts} shows the performance for such a design with three modules covering respectively low frequencies, mid-frequencies, and high frequencies, inspired from \citep{Kogut2019WP}.

Each module is based entirely on existing technologies.
After foreground subtraction, we expect to achieve limits
$|y| < 3.3\times 10^{-9}$, 
$|\mu| < 1.9\times 10^{-8}$ (95\% CL), 
and to detect the primordial hydrogen and helium recombination lines at $2\sigma$.

%----------------------------------------------
% FTS summary table
%----------------------------------------------
\begin{footnotesize}
\begin{center}
\begin{table}[]
    \caption{Multi-module absolute spectrometer; The mission sensitivity in the last column assumes 70\% useful data and a 6-year mission.}
    \vspace{5mm}
\footnotesize
    \centering
    \begin{tabular}{|l|c c c c |c|}
\hline
Module \hspace{2mm} & \hspace{2mm} $\nu_{\rm min}$ (GHz) \hspace{2mm} & \hspace{2mm} $\nu_{\rm max}$ (GHz) \hspace{2mm} & \hspace{2mm} $\Delta \nu$ (GHz)
\hspace{2mm} & \hspace{3mm} sensitivity (Jy.$\sqrt{\rm s}$) \hspace{2mm} & \hspace{2mm} mission sens. (Jy/sr) \hspace{2mm}  \\
\hline
\hline
LFM & 9.6 & 38.4 & 2.4 & 1435 & 0.12\\
MFM & 20 & 600 & 20 & 6200 & 0.54\\
HFM & 406 & 2000 & 58 & 2520 & 0.22\\
  \hline
   \end{tabular}
    \label{tab:fts}
\end{table}
\end{center}
\end{footnotesize}
%----------------------------------------------


%----------------------------------------------
% FTS summary table
%----------------------------------------------
%\begin{center}
%\begin{table}[]
%    \caption{\SPIXIE absolute spectrometer}
%    \vspace{5mm}
%\footnotesize
%    \centering
%    \begin{tabular}{l c c c c}
% \hline
%    Parameter & Units & LFM & MFM & HFM \\
%    \hline
%    Lowest Frequency 		& GHz &  9.6 & 20   & 406		\\
%    Highest Frequency		& GHz & 38.4 & 600  & 2000		\\
%    Channel Width		& GHz & 2.4  & 20   & 58		\\
%    Number of channels		& --- & 16   & 30   & 35		\\
%    Channel Sensitivity		& Jy $\sqrt$ s	& 1435 & 6200 & %2520 	\\
%  \hline
%    \end{tabular}
%    \label{tab:fts}
%\end{table}
%\end{center}
%----------------------------------------------





==> survey.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsection{CMB spectral distortions}



%A spectral coverage from about half the frequency of the tSZ minimum to twice the frequency of the tSZ maximum (70-700\,GHz) is adequate to disambiguate the various signals. 

%The main survey requirements, and their connection to the science objectives, are summarized in Table \ref{tab:STM}.

%For mapping the CMB lensing in temperature and polarization, the best observing frequency range, located between $\nu=100$ and $\nu=200$\,GHz, results from a compromise between the level of foreground contamination, the detector array sensitivity for a given focal plane size, and the angular resolution that can be achieved with a telescope of a given size. Typical deflections being of the order of $3^\prime$, we require CMB maps with an angular resolution of about $1.5^\prime$. One of the key observables for CMB lensing is the polarised signal due to the conversion of polarisaition E-modes (of even parity) into polarisation B-modes (of odd partiy). This signal is similar to polarised white noise on all angular scales larger than about $10^\prime$, at a level of 5$\mu$K.arcmin. We require full-sky polarisation observations with a noise level lower than 1$\mu$K per arcminute pixel to detect this signal at more than 5$\sigma$ in each sky pixel, at all angular scales, over the entire sky.

%Mapping the thermal SZ effect requires observations at slightly higher frequencies, covering the minimum at $ \nu\simeq 143$ and the maximum at $\nu=353$\,GHz. An angular resolution of about $1^\prime$ is required to resolve all massive clusters, at all redshifts. \textcolor{red}{[Sensitivity requirements and goals?]}

%Absolutely calibrated spectroscopy on large scale is necessary for CMB spectral distortion science, some line-intensity mapping science, for an accurate measurement of intensity on the largest angular scales (and in particular monopoles, dipoles, quadrupoles for all astrophysical components)

%\begin{table}[]
%    \caption{Survey specifications}
%\footnotesize
%    \centering
%    \begin{tabular}{|c|c|c|c|c|}
%    \hline
%         {\parbox[t]{3cm}{Observational \\ requirement}} & 
%         {\parbox[t]{3.2cm}{Frequency channels\\}} &
%         {\parbox[t]{3.5cm}{Angular resolution}} & 
%         {\parbox[t]{2.2cm}{Sensitivity}} & 
%         {\parbox[t]{1.1cm}{Sky \\ fraction}}  \\
%    \hline
%    \hline
%         {\parbox[t]{3cm}{Map the hot gas in the cosmic web}} & 
%         {\parbox[t]{3.2cm}{70-700 GHz \\ 15 channels or more}} & 
%         {\parbox[t]{3.5cm}{Req.: $1.5^\prime$; Goal: $1^\prime$; matched to clusters of $M \geq 10^{14} M_{\rm sun}$ at all $z$ }} & 
%         {\parbox[t]{2.2cm}{$\Delta y_{\rm SZ} \leq$ TBD \\ per $1^\prime$ pixel}} & 
%         {\parbox[t]{1.1cm}{100\%}}  \\
%    \hline
%         {\parbox[t]{3cm}{Map the velocity flows}} & 
%         {\parbox[t]{3.2cm}{50-400 GHz \\ 15 channels or more}} & 
%         {\parbox[t]{3.5cm}{Req.: $1.5^\prime$; Goal: $1^\prime$; matched to clusters of $M \geq 10^{14} M_{\rm sun}$ at all $z$ }} & 
%         {\parbox[t]{2.2cm}{$\Delta T_{\rm CMB} \leq$ TBD $\mu$K per $1^\prime$ pixel}} & 
%         {\parbox[t]{1.1cm}{100\%}}  \\
%    \hline
%         {\parbox[t]{3cm}{Map dark matter and measure cluster masses with CMB lensing}} & 
%         {\parbox[t]{3.2cm}{50-400 GHz \\ 15 channels or more}} & 
%         {\parbox[t]{3.5cm}{Req.: TBD; Goal: TBD; matched to deflections of $\simeq 3^\prime$}} & 
%         {\parbox[t]{2.2cm}{$\Delta T_{\rm CMB} \leq$ 2 $\mu$K per $1^\prime$ pixel for S/N$\geq$2 on B}} & 
%         {\parbox[t]{1.1cm}{100\%}}  \\
%    \hline
%    \end{tabular}
%    \label{tab:STM}
%\end{table}


\subsection{Spaceborne versus ground based observations}

